Reachability in Fixed-Dimensional Continuous VASS

Vector Addition System with States (VASS) are a ubiquitous model of infinite-state systems consisting of a set of non-negative counters which can be incremented and decremented. It is known that the reachability problem for VASS is Ackermann-complete. Because of this huge complexity, various over-approximations of VASS have been studied in the literature. One such over-approximation is continuous VASS (CVASS), in which the counters are (non-negative) rational numbers and whenever a vector is added to the current counter values, it is first scaled with an arbitrarily chosen rational factor between zero and one. It is known that the reachability problem for CVASS is $\mathsf{NP}$-complete. In this paper, we initiate the study of fixed-dimensional CVASS, i.e., CVASS with a fixed number of counters. We study both the reachability and coverability problems, under both unary and binary encodings as well as over both the non-negative and the rational semantics. This gives rise to a collection of eight different problems. As our main result, we prove a complexity dichotomy for all of these eight problems when the transition vectors are over the rationals: For dimension 1, all of the eight problems are in $\mathsf{AC}^1$, whereas for any dimension at least 2, all of the eight problems are $\mathsf{NP}$-complete. Furthermore, the hardness holds even when the underlying automaton is acyclic. To achieve this result, we present a new technique called the Egyptian prime fractions technique. Finally, we also study these problems when the transition vectors are over the integers. Except for dimension 2, we classify the complexity of these problems over the non-negative semantics: For dimension 1, all of the problems are in $\mathsf{AC}^1$, whereas for dimensions 3 and above, all of the problems are $\mathsf{NP}$-complete.

==> macros.tex <==
% % ===== PROBLEMS =====
\makeatletter
\newcommand{\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand{\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand{\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question
\NewEnviron{statement}{
  \problemtitle{}\probleminput{}\problemquestion{}% Default input is empty
  \BODY% Parse input
  \par\addvspace{.5\baselineskip}
  \noindent
  \begin{tabularx}{\columnwidth}{@{\hspace{\parindent}}X}
  \textbf{\@problemtitle}
  \\[.3\baselineskip]
  \textbf{Input:} \@probleminput \\[.2\baselineskip]
  \textbf{Question:} \@problemquestion
\end{tabularx}
  \par\addvspace{.5\baselineskip}\noindent
}
\makeatother


% \newcommand{\center}{\mathsf{center}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\centr}{\mathsf{center}}
\newcommand{\lexeq}{\leq_\mathsf{lex}}
\newcommand{\lexlt}{<_\mathsf{lex}}
\newcommand{\lexlteq}{\lexeq}
% commmands from lower bound
\newcommand{\TOWER}{\mathrm{tower}}
\newcommand{\step}{\mathsf{step}}

\DeclareMathOperator{\Reach}{Reach}
\DeclareMathOperator{\Cover}{Cover}

% Numbers
\newcommand{\nn}{\mathbb{N}}
\newcommand{\zn}{\mathbb{Z}}
\newcommand{\qn}{\mathbb{Q}}
\newcommand{\qq}{\qn}
\newcommand{\zz}{\zn}
\newcommand{\qnz}{\mathbb{Q}_{+}}
\newcommand{\zv}{\mathbf{0}}
\newcommand{\vr}[1]{\mathbf{#1}}



% Words
\newcommand{\subword}{\preceq}
\newcommand{\notsubword}{\npreceq}
\newcommand{\parikh}{\pi}

% Continuous
\newcommand{\ourboldfont}[1]{\mathbf{#1}}
\newcommand{\mach}{\mathcal{M}}
\newcommand{\graph}{\mathcal{G}}
\newcommand{\bx}{\ourboldfont{x}}
\newcommand{\by}{\ourboldfont{y}}
\newcommand{\bc}{\ourboldfont{c}}
\newcommand{\bd}{\ourboldfont{d}}
\newcommand{\bu}{\ourboldfont{u}}
\newcommand{\bv}{\ourboldfont{v}}
\newcommand{\bw}{\ourboldfont{w}}
\newcommand{\act}{\xrightarrow}
\newcommand{\actqnz}[1]{\xrightarrow[]{#1}_{\qnz}}
\newcommand{\actqn}[1]{\xrightarrow[]{#1}_{\qn}}
%\newcommand{\actqnz}[1]{\overset{#1}{\rightarrow}_{\qnz}}
%\newcommand{\actqn}[1]{\overset{#1}{\rightarrow}_{\qn}}
%\newcommand{\actqnz}[1]{\overset{#1}{\rightarrow_{\qnz}}}
%\newcommand{\actqn}[1]{\overset{#1}{\rightarrow_{\qn}}}
\newcommand{\tran}{\ourboldfont{t}}
\newcommand{\balpha}{\ourboldfont{\alpha}}
\newcommand{\bbeta}{\ourboldfont{\beta}}
\newcommand{\bgamma}{\ourboldfont{\gamma}}
\newcommand{\bdelta}{\ourboldfont{\delta}}
\newcommand{\cconf}[1]{%
    \mathchoice{\left\langle #1 \right\rangle}%
        {\langle #1 \rangle}%
        {\langle #1 \rangle}%
        {\langle #1 \rangle}%
}

% \newcommand{\center}{\mathsf{center}}
\newcommand{\NP}{\mathsf{NP}}
\newcommand{\NEXP}{\mathsf{NEXP}}
\newcommand{\PSPACE}{\mathsf{PSPACE}}
\newcommand{\NL}{\mathsf{NL}}
\newcommand{\TC}{\mathsf{TC}}
\newcommand{\AC}{\mathsf{AC}}


% trackers
\newcommand{\stTracker}[1]{\mathit{st}\mathord{(#1)}}
\newcommand{\ibt}[1]{\mathit{ibt}\mathord{(#1)}}
\newcommand{\sumt}[1]{\mathit{sumt}\mathord{(#1)}}

% Lifting
\newcommand{\far}{\mathit{far}}
\newcommand{\lar}{\mathit{lar}}
\newcommand{\wbgn}{\mathit{begin}}
\newcommand{\wend}{\mathit{end}}
\newcommand{\extra}{\mathit{extra}}

% Language classes
\newcommand{\cC}{\mathcal{C}}

\newcommand{\inte}[0]{\mathcal{I}}

%\DeclareMathOperator{\exp}{exp}



% Comments
\newcommand{\RM}[1]{\todo[inline]{\textcolor{white}{\textbf{RM}: #1}}}
\newcommand{\rst}[1]{\todo[inline]{\textcolor{white}{\textbf{RST}: #1}}}
\newcommand{\mh}[1]{\todo[inline]{\textcolor{white}{\textbf{MH}: #1}}}
\newcommand{\balain}[1]{\todo[inline]{\textcolor{white}{\textbf{BA}: #1}}}
\newcommand{\gz}[1]{\todo[inline]{\textbf{GZ}: #1}}

\newcommand{\bala}[1]{\todo{\textcolor{white}{\textbf{BA}: #1}}}
\newcommand{\lukasz}[1]{\todo{\textcolor{black}{\textbf{ŁU}: #1}}}
\newcommand{\michal}[1]{\todo{\textcolor{gray}{\textbf{MA}: #1}}}


\newcommand{\weight}[1]{W(#1)}
\newcommand{\fl}[1]{\mathsf{flat}(#1)}


\newcommand{\myparagraph}[1]{\vspace{0.2cm}\noindent\textbf{#1.} }




\newcommand{\transitions}{\ensuremath{T}}

\newcommand{\calO}{O}




%tikz
\usepackage{tikz}
\usepackage[justification=centering]{caption}

\tikzstyle{loop above}=[tran, to path={.. controls +(60:1) 
	and +(120:1) .. (\tikztotarget) \tikztonodes}]
\tikzstyle{loop below}=[tran, to path={.. controls +(240:1) 
	and +(300:1) .. (\tikztotarget) \tikztonodes}]
\tikzstyle{loop left}=[tran,  to path={.. controls +(150:1) 
	and +(210:1) .. (\tikztotarget) \tikztonodes}]
\tikzstyle{loop right}=[tran,  to path={.. controls +(330:1) 
	and +(30:1) .. (\tikztotarget) \tikztonodes}]

\tikzstyle{state}=[circle,,draw,minimum size=4ex,inner sep=0pt,font=\large, very thick,text centered, fill=blue!20, fill opacity=0.2, draw=black!80, text opacity=1]

\tikzstyle{bigtran}=[very thick,draw,-angle 60,font=\scriptsize, inner sep = 6pt]
\tikzstyle{tran}=[thick,draw,->,>=stealth,rounded corners]
\tikzstyle{tran right above}=[tran, to path={.. controls +(60:.8) and +(120:.8) .. (\tikztotarget) \tikztonodes}]
\tikzstyle{tran left above}=[tran, to path={.. controls +(120:.8) and +(60:.8) .. (\tikztotarget) \tikztonodes}]
\tikzstyle{tran left below}=[tran, to path={.. controls +(240:.8) and +(300:.8) .. (\tikztotarget) \tikztonodes}]
\tikzstyle{tran right below}=[tran, to path={.. controls +(300:.8) and +(240:.8) .. (\tikztotarget) \tikztonodes}]
\tikzstyle{loop right below}=[tran, to path={.. controls +(330:.8) and +(270:.8) .. (\tikztotarget) \tikztonodes}]
\tikzstyle{loop right above}=[tran, to path={.. controls +(30:.8) and +(90:.8) .. (\tikztotarget) \tikztonodes}]


%automata
\newcommand{\aut}[1]{\mathcal{#1}}
\newcommand{\trans}[1]{\xrightarrow{#1}}



%prevent footnote from splitting voer multiple pages
\interfootnotelinepenalty=10000




\usepackage{tcolorbox}
